Comparable Corpora: Opportunities for New Research Directions

Most conference papers present new results, but this paper will focus more on opportunities for the audience to make their own contributions. This paper is intended to challenge the community to think more broadly about what we can do with comparable corpora. We will start with a review of the history, and then suggest new directions for future research. This was a keynote at BUCC-2025, a workshop associated with Coling-2025.

==> notes.tex <==
when do you need what?

how much time will I have for my talk?

You mentioned an opportunity to contribute up to 8 pages to the proceedings

I was thinking of a title like

title: Comparable Corpora: An Opportunity to Study Differences as Well as Similarities

do you want a short abstract sooner?  when do you need the paper?

I would like to use this as an opportunity to give the audience opportunities of things to work on, rather than plug my own "successes"

You may remember EMNLP was in Hong Kong just before COVID.  I was interested in the coverage of demonstrations in Hong Kong.  The story was very simple in New York and in Beijing.  They didn't see it the same way, but the story was simple in both places.  Then when I went to Hong Kong for EMNLP, the story was much more complicated.  I think we all have a tendency to oversimplify the truth, especially for things that are not so close to us.

There is that famous cover of the New Yorker: https://en.wikipedia.org/wiki/View_of_the_World_from_9th_Avenue

I'd like to challenge the community to think more broadly about what we can do with comparable corpora.

I'm attaching a paper Omar and I just submitted to SIGIR Forum.   I'd like to expand on section 8, especially the story about the dress:

In more recent work (Mohamed et al. [2024]), we have been trying to move past unambiguous objective labels by asking annotators to add emotion labels and captions in 28 languages to WikiArt. For a particular portrait, many annotators thought the woman was beautiful but some objected to her dress as too revealing. One reviewer insisted on an ethics review, objecting to the objection to the dress. We object to the objection to the objection; it is inappropriate to impose our views on the rest of the world. We are not siding with one annotator over another, but rather than remove bias from corpora, we hope to build bots that will be more aware of regional sensitivities to topics such as: dress, religion and alcohol. In addition to publishing a benchmark, we offer baseline implementations of captioning systems. Hopefully, the community will accept the challenge and come up with even better systems that embrace diversity over many regions, cultures and languages. 

I would also like to challenge our view about what comparable corpora are.
multimedia: we normally think about comparable corpora as different news stories about similar events (in different languages), or different wikipedia articles about similar topics (in different languages).  What about different modalities: audio, pictures, video; see https://aclanthology.org/2024.emnlp-main.1165/, for example
Semantic Scholar has lots of papers in lots of languages, with a citation graph.  We can easily find papers that are near one another in the graph, but not in the same language.  Can we compare and contrast them?  I have tried to use RAG to compare and contrast papers that are similar to one another in terms of academic recommendations, but it should be possible to do better than I have done; see section 3.4 of https://www.cambridge.org/core/services/aop-cambridge-core/content/view/4FF461F4066A0C16135F2D2849E3356A/S1351324924000044a.pdf/emerging-trends-a-gentle-introduction-to-rag.pdf

